From Words to Code: Harnessing Data for Program Synthesis from Natural Language

Creating programs to correctly manipulate data is a difficult task, as the underlying programming languages and APIs can be challenging to learn for many users who are not skilled programmers. Large language models (LLMs) demonstrate remarkable potential for generating code from natural language, but in the data manipulation domain, apart from the natural language (NL) description of the intended task, we also have the dataset on which the task is to be performed, or the "data context". Existing approaches have utilized data context in a limited way by simply adding relevant information from the input data into the prompts sent to the LLM. In this work, we utilize the available input data to execute the candidate programs generated by the LLMs and gather their outputs. We introduce semantic reranking, a technique to rerank the programs generated by LLMs based on three signals coming the program outputs: (a) semantic filtering and well-formedness based score tuning: do programs even generate well-formed outputs, (b) semantic interleaving: how do the outputs from different candidates compare to each other, and (c) output-based score tuning: how do the outputs compare to outputs predicted for the same task. We provide theoretical justification for semantic interleaving. We also introduce temperature mixing, where we combine samples generated by LLMs using both high and low temperatures. We extensively evaluate our approach in three domains, namely databases (SQL), data science (Pandas) and business intelligence (Excel's Power Query M) on a variety of new and existing benchmarks. We observe substantial gains across domains, with improvements of up to 45% in top-1 accuracy and 34% in top-3 accuracy.

==> figs/spider-kaggle-few-shot-cosine-table.tex <==
% Read data from CSV file and store it in a table
\pgfplotstableread[col sep=comma]{data/spider-kaggle-few-shot-cosine.csv}\loadedtable

% Create a new column 'tempForDisplay' in the table
\pgfplotstablecreatecol[
    create col/assign/.code={
        \edef\newentry{%
            \ifnum\pgfplotstablerow=0
                \thisrow{temp} % If first row, display the temperature value
            \else
                \ifnum\pdfstrcmp{\prevrow{temp}}{\thisrow{temp}}=0
                    ~ % If the temperature value is the same as the previous row, display nothing
                \else
                    \thisrow{temp} % Otherwise, display the temperature value
                \fi
            \fi
        }%
        \pgfkeyslet{/pgfplots/table/create col/next content}\newentry
    }
]{tempForDisplay}\loadedtable

% Begin table environment
\begin{table}[]
    % Typeset the table with specified column styles and formatting
    \pgfplotstabletypeset[
        % Define a style for displaying values with percentage
        values style/.style={
            precision=1,
            fixed zerofill,
            fixed,
            column type=c,
            postproc cell content/.append code={
               \pgfkeysalso{@cell content/.add={}{}}%
            },
        },
        % Give us the ability to throw ome extra midrules in here
        midrule/.style={
            every row no #1/.style={
                before row=\midrule
            }
        },
        midrule=4,
        midrule=8,
        midrule=12,
        % Define column styles and names
        columns={tempForDisplay,k,spiderEXE,spiderEXA,kaggleEXE,kaggleEXA},
        columns/tempForDisplay/.style={
            column name=Temp.,
            column type=l,
            string type
        },
        columns/spiderEXE/.style={column name=Execution, values style},
        columns/spiderEXA/.style={column name=Exact, values style},
        columns/kaggleEXE/.style={column name=Execution, values style},
        columns/kaggleEXA/.style={column name=Exact, values style},
        % Define header row style
        every head row/.style={
            before row={%
                \toprule & & \multicolumn{2}{c}{Spider} & \multicolumn{2}{c}{Kaggle} \\ 
                \cmidrule(lr){3-4} \cmidrule(lr){5-6}
            },
            after row={\midrule}
        },
        % Define last row style
        every last row/.style={after row=\bottomrule},
        % Add midrule for every row where tempForDisplay is not empty
        every row/.append style={
            before row={%
                \ifnum\pdfstrcmp{\thisrow{tempForDisplay}}{~}=0
                \else
                    \midrule
                \fi
            },
        },
    ]{\loadedtable}
    % Caption and such
    \caption{Few-shot with dynamic training examples (cosine) \jjh{How many few-shots? Same Q for the other few-shot static table} \sd{3 for everything}}
    \label{tab:fewshot:dynamic}
\end{table}

==> figs/spider-kaggle-few-shot-static-table.tex <==
% Read data from CSV file and store it in a table
\pgfplotstableread[col sep=comma]{data/spider-kaggle-few-shot-static.csv}\loadedtable

% Create a new column 'tempForDisplay' in the table
\pgfplotstablecreatecol[
    create col/assign/.code={
        \edef\newentry{%
            \ifnum\pgfplotstablerow=0
                \thisrow{temp} % If first row, display the temperature value
            \else
                \ifnum\pdfstrcmp{\prevrow{temp}}{\thisrow{temp}}=0
                    ~ % If the temperature value is the same as the previous row, display nothing
                \else
                    \thisrow{temp} % Otherwise, display the temperature value
                \fi
            \fi
        }%
        \pgfkeyslet{/pgfplots/table/create col/next content}\newentry
    }
]{tempForDisplay}\loadedtable

% Begin table environment
\begin{table}[]
    % Typeset the table with specified column styles and formatting
    \pgfplotstabletypeset[
        % Define a style for displaying values with percentage
        values style/.style={
            precision=1,
            fixed zerofill,
            fixed,
            column type=c,
            postproc cell content/.append code={
               \pgfkeysalso{@cell content/.add={}{}}%
            },
        },
        % Give us the ability to throw ome extra midrules in here
        midrule/.style={
            every row no #1/.style={
                before row=\midrule
            }
        },
        midrule=4,
        midrule=8,
        midrule=12,
        % Define column styles and names
        columns={tempForDisplay,k,spiderEXE,spiderEXA,kaggleEXE,kaggleEXA},
        columns/tempForDisplay/.style={
            column name=Temp.,
            column type=l,
            string type
        },
        columns/spiderEXE/.style={column name=Execution, values style},
        columns/spiderEXA/.style={column name=Exact, values style},
        columns/kaggleEXE/.style={column name=Execution, values style},
        columns/kaggleEXA/.style={column name=Exact, values style},
        % Define header row style
        every head row/.style={
            before row={%
                \toprule & & \multicolumn{2}{c}{Spider} & \multicolumn{2}{c}{Kaggle} \\ 
                \cmidrule(lr){3-4} \cmidrule(lr){5-6}
            },
            after row={\midrule}
        },
        % Define last row style
        every last row/.style={after row=\bottomrule},
        % Add midrule for every row where tempForDisplay is not empty
        every row/.append style={
            before row={%
                \ifnum\pdfstrcmp{\thisrow{tempForDisplay}}{~}=0
                \else
                    \midrule
                \fi
            },
        },
    ]{\loadedtable}
    % Caption and such
    \caption{Few-shot with static training examples \eat{\jjh{We should not show temp=0 k>1, you're just seeing variance based on floating point errors on the GPUs the model is running on... in ``theory'' it's deterministic at temp=0 and all k>1 results are the same} \sd{Agreed. All of the data currently in the document here (for NL to SQL) is a brain-dead dump of what we have. Nothing has been sifted through or analyzed to make a coherent story. All of this will be ironed out in the coming days.}}}
    \label{tab:fewshot:static}
\end{table}

==> repair.tex <==
\section{Program Repair}
\label{sec:repair}

Owner: Anirudh.

Describe the details of the repair techniques. 


    \begin{itemize}
        \item Creating the repair prompts (choosing candidate repair programs/their common components, candidate outputs...)
        
        \item Using existing PBE systems (flash fill) and their incorporation in the repair pipeline.  
    \end{itemize}


